Online Learning in Contextual Second-Price Pay-Per-Click Auctions

We study online learning in contextual pay-per-click auctions where at each of the $T$ rounds, the learner receives some context along with a set of ads and needs to make an estimate on their click-through rate (CTR) in order to run a second-price pay-per-click auction. The learner's goal is to minimize her regret, defined as the gap between her total revenue and that of an oracle strategy that always makes perfect CTR predictions. We first show that $\sqrt{T}$-regret is obtainable via a computationally inefficient algorithm and that it is unavoidable since our algorithm is no easier than the classical multi-armed bandit problem. A by-product of our results is a $\sqrt{T}$-regret bound for the simpler non-contextual setting, improving upon a recent work of [Feng et al., 2023] by removing the inverse CTR dependency that could be arbitrarily large. Then, borrowing ideas from recent advances on efficient contextual bandit algorithms, we develop two practically efficient contextual auction algorithms: the first one uses the exponential weight scheme with optimistic square errors and maintains the same $\sqrt{T}$-regret bound, while the second one reduces the problem to online regression via a simple epsilon-greedy strategy, albeit with a worse regret bound. Finally, we conduct experiments on a synthetic dataset to showcase the effectiveness and superior performance of our algorithms.

==> synthetic.tex <==
\subsection{Synthetic Data}\label{sec:synthetic_data}
\begin{figure}[t]
  \centering
  \includegraphics[width=0.49\textwidth]{Regret_synthetic.png}
  \caption{Performance of different algorithms on synthetic dataset}
  \label{fig:regret_synthetic}
\end{figure}

\paragraph{Dataset.} In this experiment, we generate $T=10000$ auction data with each sample of format $\{(X_t, b_t,M_t)\}_{t=1}^T$. The number of bidders $N_t$ at each round $t$ is uniformly sampled from $5$ to $10$. For each data point $(X_t,b_t)$, each entry of the bid at each round $b_t\in [0,1]^{N_t}$ is sampled uniformly from $[0.1,1]$. $X_t\in\R^{N_t\times 2d}$ represents the context with $d=128$. Denoting $X_{t,i}$ to be the $i$-th column vector of $X_t$. The sub-vector formed by the first $d$ entries of each column $X_i$'s is the same, which represents the $d$-dimensional embedding of the user query and the second half of each $X_{t,i}$ represents the $d$-dimensional embedding of the $i$-th participating ads feature.

\paragraph{Function class $\calF$.} In our experiments, we consider the following function class.
\begin{align}\label{eqn:func_class}
    \calF &= \{f:f(X,i)=\sigmoid(\theta^\top X_i), \theta\in [-1,1]^{2d}\},
\end{align}
where for any $u\in \R$, $\sigmoid(u)=\frac{1}{1+e^{-u}}$. We generate the true CTR for each bidder with context $X_i$ by first assigning a random CTR uniformly chosen from $[0.2,1]$ and then using the full dataset to fit the model $f^*\in \calF$. We treat the CTR predicted by $f^*$ as the true CTR. To avoid trivial strategies, such as predicting a constant CTR for each bidder at each round, work well, for each round $t$, we reset the bid to be $2$ for the bidder with the lowest true CTR value.

\paragraph{Experiment configurations and results.} For \pref{alg:EXP4} with \optsq, the parameter $\eta$ is chosen from $\{\frac{1}{16}, \frac{1}{8}, \frac{1}{4}\}$ and the SGLD sampling step size is chosen from $\{0.001,0.005,0.01,0.05\}$. For \pref{alg:squareCB.A}, the parameter $\epsilon$ is chosen from $\{T^{-\frac{1}{3}}, 2T^{-\frac{1}{3}}, 4T^{-\frac{1}{3}}\}$. We run both \pref{alg:EXP4} with \optsq and \pref{alg:squareCB.A} with $4$ different random seeds under different hyper-parameter choices and report the average and the standard deviation of the cumulative regret over these $4$ trials under the best hyper parameter tuning. \pref{fig:regret_synthetic} shows our empirical results. We can see that \pref{alg:EXP4} with \optsq (blue curve) and \pref{alg:squareCB.A} (green curve) both achieves favorable regret with \pref{alg:EXP4} with \optsq outperforming \pref{alg:squareCB.A}. We also implement a version of \pref{alg:EXP4} with \optsq but without the optimistic term $\smax_j f(x_t,j)b_{t,j}$ (orange curve). Similar to~\citep{zhang2022feel}, the result shows the importance of including this optimistic term in the loss estimator construction without this term. In addition, we implement two baseline algorithms. The first algorithm ``Fixed CTR'' predicts a constant CTR at each round for each bidder. With this approach, the learner will always pick the ad with the highest bid. The second algorithm predicts a random CTR at each round for each bidder. We show that both algorithms perform worse than our proposed algorithm and achieve linear regret.
